Improving Object Detection by Label Assignment Distillation

Label assignment in object detection aims to assign targets, foreground or background, to sampled regions in an image. Unlike labeling for image classification, this problem is not well defined due to the object's bounding box. In this paper, we investigate the problem from a perspective of distillation, hence we call Label Assignment Distillation (LAD). Our initial motivation is very simple, we use a teacher network to generate labels for the student. This can be achieved in two ways: either using the teacher's prediction as the direct targets (soft label), or through the hard labels dynamically assigned by the teacher (LAD). Our experiments reveal that: (i) LAD is more effective than soft-label, but they are complementary. (ii) Using LAD, a smaller teacher can also improve a larger student significantly, while soft-label can't. We then introduce Co-learning LAD, in which two networks simultaneously learn from scratch and the role of teacher and student are dynamically interchanged. Using PAA-ResNet50 as a teacher, our LAD techniques can improve detectors PAA-ResNet101 and PAA-ResNeXt101 to $46 \rm AP$ and $47.5\rm AP$ on the COCO test-dev set. With a stronger teacher PAA-SwinB, we improve the students PAA-ResNet50 to $43.7\rm AP$ by only 1x schedule training and standard setting, and PAA-ResNet101 to $47.9\rm AP$, significantly surpassing the current methods. Our source code and checkpoints are released at https://git.io/JrDZo.

==> Tex/sup_experiment.tex <==
\subsection{Deformable Convolution}
We conduct experiments with the model using Deformable Convolution Network (DCN) backbone ResNeXt-64x4d-101-DCN. 
%We also perform multi-scale testing adopted in ATSS[16], that is, with 12 scales and flipping augmentation on the test images.

\begin{table}[!h]
\caption{Compare with State-of-the-art methods (single model) on MS COCO \textit{test} set with 2x schedule (180k iters). (*) denotes that DCN is applied to 3 levels P3-P5. Bold text means the best performance.}
\label{tab:supSOTA}
\centering
\begin{adjustbox}{max width=\columnwidth}
		\begin{tabular}{|l|l|l|l|l|l|l|}
			\hline
			\multicolumn{1}{|l|}{\textbf{Method}} & \multicolumn{1}{l|}{\textbf{AP}} & \multicolumn{1}{l|}{\textbf{AP$_{\textbf{50}}$}} & \multicolumn{1}{l|}{\textbf{AP$_{\textbf{75}}$}} & \multicolumn{1}{l|}{\textbf{AP$_\textbf{S}$}} & \multicolumn{1}{l|}{\textbf{AP$_\textbf{M}$}} & \multicolumn{1}{l|}{\textbf{AP$_\textbf{L}$}} \\ \hline
			\multicolumn{7}{|l|}{\textbf{ResNeXt-64x4d-101-DCN}}\\                                                  
				SAPD[19]                                  & 47.4                             & 67.4                               & 51.1                               & 28.1                              & 50.3                              & 61.5                              \\
				ATSS[16]                                   & 47.7                             & 66.5                               & 51.9                               & 29.7                              & 50.8                              & 59.4                              \\
				A.Assign[18]                                   & 48.3                             & 67.4                               & 52.7                               & 29.2                              & 51.0                              & 60.3                              \\
				PAA[9]                                   & 49.0                             & 67.8                               & 53.3                               & 30.2                              & 51.3                              & 62.2                              \\
				OTA[6]                                   & \textbf{49.2}                             & 67.6                               & 53.5                               & 30.3                              & \textbf{52.5}                              & \textbf{62.3}                              \\
				IQDet[13]                                 & 49.0                             & 67.5                               & 53.1                               & 30.0                              & 52.3                              & 62.0                              \\
				\textbf{CoLAD[ours]*}                                &     49.1                             &         \textbf{68.2}                           &      \textbf{53.9 }                             &       \textbf{30.8}                            &       \textbf{52.5}                            &	  61.9                            \\ \hline  
%				\multicolumn{7}{|l|}{\textbf{ResNeXt-64x4d-101-DCN} - Multi-scale testing}\\ 
%				ATSS{[}16{]}     & 50.7 & 68.9 & 56.3 & 33.2 & 52.9 & 62.2 \\ 
%				PAA{[}9{]}       & 51.4 & 69.7 & 57.0 & 34.0 & 53.8 & 64.0 \\ 
%				A.Assign{[}18{]} & 52.1 & 69.6 & 58.0 & 33.9 & 54.0 & 64.0 \\ 
%				OTA{[}6{]}       & 51.5 & 68.6 & 57.1 & 34.1 & 53.7 & 64.1 \\ 
%				IQDet{[}13{]}    & 51.6 & 68.7 & 57.0 & 34.5 & 53.6 & 64.5 \\ 
%%				CoLAD {[}ours{]} & 50.8 & 68.8 & 56.3 & 34.5 & 53.6 & 61.8 \\ \hline 
% 				\textbf{CoLAD[ours]*} & & & & & & \\ \hline 
	\end{tabular}
\end{adjustbox}
\end{table}
As shown in \tab{supSOTA}, with DCN applied on the P3-P5 levels, CoLAD can significantly improve the AP for small and medium objects ($+0.6 \rm AP_S$ and $+1.2 \rm AP_M$), and the localization quality ($+0.6 \rm AP_{75}$), but not on the large objects ($-0.3 \rm AP_L$) relatively to the baseline PAA. The final result is $0.1 \rm AP$ less than OTA, which hence implies the bias toward $\rm AP_L$. We will add the experiment with DCN applied only to P4-P5 levels for better comparison with the others.  


\subsection{Improvement on Teacher}
We inspect the teacher PAA-R50 's performance after trained with CoLAD in the SOTA test. As shown in \Tab{TeacherSOTA}, the performance is almost equivalent in the three cases.
\begin{table}[!h]
	\caption{Evaluate the teacher ResNet-50 after being co-trained with different students: ResNet-101 (R101), ResNeXt-64x4d-101(X101), and ResNeXt-64x4d-101-DCN (X101-DCN), on the MS COCO \textit{test} set.}
	\label{tab:TeacherSOTA}
\begin{adjustbox}{max width=\columnwidth}
	\small{
		\begin{tabular}{|l|l|l|l|l|l|l|}
			\hline
			\multicolumn{1}{|l|}{\textbf{Students}} & \multicolumn{1}{l|}{\textbf{AP}} & \multicolumn{1}{l|}{\textbf{AP$_{\textbf{50}}$}} & \multicolumn{1}{l|}{\textbf{AP$_{\textbf{75}}$}} & \multicolumn{1}{l|}{\textbf{AP$_\textbf{S}$}} & \multicolumn{1}{l|}{\textbf{AP$_\textbf{M}$}} & \multicolumn{1}{l|}{\textbf{AP$_\textbf{L}$}} \\ \hline
			- & 43.8 & 61.8 & 47.8 & 26.4 & 47.1 & 54.5 \\ 
			R101          & 44.7 & 62.9 & 49.0 & 27.4 & 48.2 & 55.0 \\ 
			X101          & \textbf{44.8} & 63.0 & \textbf{49.1} & \textbf{27.7} & \textbf{48.3} & 54.8 \\ 
			X101-DCN      & \textbf{44.8} & \textbf{63.1} & 49.0 & 27.6 & 48.2 & \textbf{55.3} \\ \hline         
		\end{tabular}}
	\end{adjustbox}
\end{table}

==> Tex/visualization.tex <==
\subsection{Examine Prediction Quality}
We compare the prediction quality of the student PAA-R101 and teacher PAA-R50 using CoLAD in term of $\rm AP$ for each individual image. \Fig{compareTS} shows their predictions on several samples. We see that their predicted bounding boxes are closely matched, with minor difference on class confidence prediction. 
\begin{figure*}
	\centering
	\setlength{\lineskip}{0pt}
	\begin{minipage}[t]{0.32\linewidth}
		\includegraphics[width=1.\linewidth,height=0.8\linewidth]{Fig/vis/1s.png}\hfill
		\includegraphics[width=1.\linewidth,height=0.8\linewidth]{Fig/vis/1t.png}\hfill
		\includegraphics[width=1.\linewidth,height=0.8\linewidth]{Fig/vis/2s.png}\hfill
		\includegraphics[width=1.\linewidth,height=0.8\linewidth]{Fig/vis/2t.png}\hfill
	\end{minipage}% 
	\begin{minipage}[t]{0.32\linewidth}
		\includegraphics[width=1.\linewidth,height=0.8\linewidth]{Fig/vis/7s.png}\hfill
		\includegraphics[width=1.\linewidth,height=0.8\linewidth]{Fig/vis/7t.png}\hfill
		\includegraphics[width=1.\linewidth,height=0.8\linewidth]{Fig/vis/3s.png}\hfill
		\includegraphics[width=1.\linewidth,height=0.8\linewidth]{Fig/vis/3t.png}\hfill
	\end{minipage}% 
	\begin{minipage}[t]{0.32\linewidth}
		\includegraphics[width=1.\linewidth,height=0.8\linewidth]{Fig/vis/5s.png}\hfill
		\includegraphics[width=1.\linewidth,height=0.8\linewidth]{Fig/vis/5t.png}\hfill
		\includegraphics[width=1.\linewidth,height=0.8\linewidth]{Fig/vis/8s.png}\hfill
		\includegraphics[width=1.\linewidth,height=0.8\linewidth]{Fig/vis/8t.png}\hfill
	\end{minipage}% 
	
	\caption{Visualize prediction results of the teacher PAA-R50 (odd rows) and Student PAA-R101 (even rows) trained with CoLAD.}
	\label{fig:compareTS}
\end{figure*}

\subsection{Positive Anchor Visualization}
\Fig{anchor} visualizes the positive anchors of the model PAA-ResNet50, trained with the baseline PAA and CoLAD at the early (epoch 1), middle (epoch 6), and the later (epoch 12) training progress, respectively. We see that they are both assigned dynamically, dependent on each object, and tend to be near the centers. 
\begin{figure*}
	\centering
	\setlength{\lineskip}{0pt}
	\begin{minipage}[t]{0.32\linewidth}
		\includegraphics[width=1.\linewidth,height=0.5\linewidth]{Fig/anchor/73_base_paa_x50_e0.png}\hfill
		\includegraphics[width=1.\linewidth,height=0.5\linewidth]{Fig/anchor/73_cl_fisher_e0.png}\hfill
%		\includegraphics[width=1.\linewidth,height=0.7\linewidth]{Fig/anchor/246_base_e0.png}\hfill
%		\includegraphics[width=1.\linewidth,height=0.7\linewidth]{Fig/anchor/246_co_e0.png}\hfill
		\includegraphics[width=1.\linewidth,height=0.7\linewidth]{Fig/anchor/306_base_e0.png}\hfill
		\includegraphics[width=1.\linewidth,height=0.7\linewidth]{Fig/anchor/306_co_e0.png}\hfill
	\end{minipage}% 
	\begin{minipage}[t]{0.32\linewidth}
		\includegraphics[width=1.\linewidth,height=0.5\linewidth]{Fig/anchor/73_base_paa_x50_e6.png}\hfill
		\includegraphics[width=1.\linewidth,height=0.5\linewidth]{Fig/anchor/73_cl_fisher_e6.png}\hfill
%		\includegraphics[width=1.\linewidth,height=0.7\linewidth]{Fig/anchor/246_base_e6.png}\hfill
%		\includegraphics[width=1.\linewidth,height=0.7\linewidth]{Fig/anchor/246_co_e0.png}\hfill
		\includegraphics[width=1.\linewidth,height=0.7\linewidth]{Fig/anchor/306_base_e6.png}\hfill
		\includegraphics[width=1.\linewidth,height=0.7\linewidth]{Fig/anchor/306_co_e0.png}\hfill
	\end{minipage}% 
	\begin{minipage}[t]{0.32\linewidth}
		\includegraphics[width=1.\linewidth,height=0.5\linewidth]{Fig/anchor/73_base_paa_x50_e12.png}\hfill
		\includegraphics[width=1.\linewidth,height=0.5\linewidth]{Fig/anchor/73_cl_fisher_e12.png}\hfill
%		\includegraphics[width=1.\linewidth,height=0.7\linewidth]{Fig/anchor/246_base_e12.png}\hfill
%		\includegraphics[width=1.\linewidth,height=0.7\linewidth]{Fig/anchor/246_co_e12.png}\hfill
		\includegraphics[width=1.\linewidth,height=0.7\linewidth]{Fig/anchor/306_base_e12.png}\hfill
		\includegraphics[width=1.\linewidth,height=0.7\linewidth]{Fig/anchor/306_co_e12.png}\hfill
	\end{minipage}% 
	\caption{Positive anchors assigned in PAA-R50 baseline (odd rows) and PAA-R50 with CoLAD (even rows) during the training progress: epoch 1, 6, and 12 are shown in the left, middle, and right columns, respectively. Positive anchors at the FPN level P3-P7 are represented by Orange, Magenta, Red, Green, Blue, respectively.}
	\label{fig:anchor}
\end{figure*}

\
